Restricted Bayesian Neural Network

Modern deep learning tools are remarkably effective in addressing intricate problems. However, their operation as black-box models introduces increased uncertainty in predictions. Additionally, they contend with various challenges, including the need for substantial storage space in large networks, issues of overfitting, underfitting, vanishing gradients, and more. This study explores the concept of Bayesian Neural Networks, presenting a novel architecture designed to significantly alleviate the storage space complexity of a network. Furthermore, we introduce an algorithm adept at efficiently handling uncertainties, ensuring robust convergence values without becoming trapped in local optima, particularly when the objective function lacks perfect convexity.

==> extra.tex <==
\begin{theorem}[Convergence of RBNN]
    RBNN algorithm almost surely converges to global optimum point as $t \to \infty$
\end{theorem}

\begin{proof}
In RBNN, we can say that our algorithm has converged when the weights do not change. Now the weight $W^{l}~\forall 1\leq l\leq L$ will not change if the distribution parameters $\mu$ and $\sigma$ reach such a point that a constant value is sampled at each epoch. If $\mu$ and $\sigma$ is fixed to $m$ and $s$ respectively and always samples fixed weights $W^{l}~\forall 1\leq l\leq L \implies~E(h_{s}(x))$ then we can say the algorithm has converged. Thus, on sorting and considering first $\rho$ samples and updating $\mu$ and $\sigma$ will not affect the old $\mu$ and $\sigma$ values.

However, now we need to show that this point is $\epsilon$ close to optimum point, To prove this let us consider that our parameters have reached convergence but that point is not $\epsilon$ close to optimal point. Needless to say that unless it is an optimal point, the error function $~E(h_{s}(x))>0$. If the error value exists the update equation given by $\mu_{(j+1)} = \alpha \underset{k \in M}{\Sigma}\frac{f(X_{k})X_{k}}{\underset{k \in M}{\Sigma}f(X_{k})} + (1-\alpha) * v_{j}$ will get updated. But then it contradicts the fact that distribution parameters have converged. Thus, if the distribution parameters converge to a point, it has to be the optimum point.
\end{proof}

We trained our model on two standard datasets: the IRIS dataset and the Pulsar-star dataset. The loss plots of our model were compared with those of standard feed-forward neural networks (FFNN) and Bayesian neural networks (BNN), as illustrated in Figures \ref{fig:pul_comp} and \ref{fig:iris_comp}. The Pulsar dataset, containing nearly twenty-thousand data samples, had missing data columns, which were removed, resulting in 12528 data samples for our experiments. The observations from this experiment are as follows:

For the Pulsar dataset:
1. The Restricted Bayesian Neural Network (RBNN) model demonstrated greater efficiency in terms of storage space and accuracy compared to FFNN and BNN. Within 10 epochs, the loss in RBNN approached almost zero.
2. The accuracy achieved using RBNN on a subset of the dataset was nearly 93%, whereas it was approximately 91% and 90% for FFNN and BNN, respectively.
3. The storage space required for RBNN was also less compared to FFNN and BNN. RBNN only required storing the means, while FFNN needed to store the complete weights, and BNN required storing means and standard deviations associated with each connection.

For the IRIS dataset:
1. The RBNN model initially had a higher error compared to BNN and FFNN due to randomly sampled weights. However, after training for a few epochs (specifically 10 epochs), our model proved more efficient.
2. The accuracy obtained after testing on a subset of the dataset (10 samples) showed RBNN achieving an accuracy of 99.3%, while FFNN and BNN achieved accuracies of 95.8% and 92.6%, respectively.
3. The storage space required for RBNN was also less compared to FFNN and BNN, with RBNN only requiring the storage of means.

A detailed comparison and analysis of the results for the three models are presented in Table \ref{comp_table1} and Table \ref{comp_table2}.

